IAC: A Framework for Enabling Patient Agency in the Use of AI-Enabled Healthcare

In healthcare, the role of AI is continually evolving, and understanding the challenges its introduction poses on relationships between healthcare providers and patients will require a regulatory and behavioral approach that can provide a guiding base for all users involved. In this paper, we present IAC (Informing, Assessment, and Consent), a framework for evaluating patient response to the introduction of AI-enabled digital technologies in healthcare settings. We justify the need for IAC with a general introduction of the challenges with and perceived relevance of AI in human-welfare-centered fields, with an emphasis on the provision of healthcare. The framework is composed of three core principles that guide how healthcare practitioners can inform patients about the use of AI in their healthcare, how practitioners can assess patients' acceptability and comfortability with the use of AI, and how patient consent can be gained after this process. We propose that the principles composing this framework can be translated into guidelines that improve practitioner-patient relationships and, concurrently, patient agency regarding the use of AI in healthcare while broadening the discourse on this topic.

==> tables.tex <==
\begin{table*}[ht]
\caption{AI Typology}
\begin{center}
\begin{tabular}{lllll}
% \cline{1-3} \vspace{0.1 cm}
\ & \textbf{Administrative} & \textbf{Diagnostic} &  &  \\ 
\cline{1-3}
\multicolumn{1}{|l|}{\textbf{Patient-facing}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}
  \begin{itemize}
    \item Virtual Assistants for waiting rooms
    \item Health monitoring
    \item Medication management
    \item AI-driven robots assisting with care
  \end{itemize}
  \end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}
  \begin{itemize}
    \item Computer-aided diagnosis (CADx, image processing)
    \item Digital consultations (clinical decision support systems, CDS)
    \item Brain-Computer interfaces (BCI) - Group-level disease prevention
    \item Individualized precision medicine (with AI)
    \item Robot-assisted surgery
  \end{itemize}
  \end{tabular}} &
   &
   \\ \cline{1-3}
\multicolumn{1}{|l|}{\textbf{Non patient-facing}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}
    \begin{itemize}
        \item Bed allocations
        \item Scanning of Electronic Patient Records
        \item Staffing optimization: level and hiring
        \item Simulations for Medical Education
        \item Forecasting demand for medical resources
        \item Fraud detection
        \item Cybersecurity for health data
    \end{itemize}
    \end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}
  \begin{itemize}
    \item Medical research and drug discovery (e.g. electrophysiology)
    \item Analyzing clinical laboratory results
  \end{itemize}
  \end{tabular}} &
   &
   \\ \cline{1-3}
 &                         &                     &  &  \\
 \multicolumn{5}{l}{Note: based on \cite{jiang2017artificial}, \cite{arora2020conceptualising} and \cite{kalis201810}. }
\end{tabular}
\end{center}
\end{table*}
% Table + Caption -- Sources: Authors’ elaboration based on Artificial intelligence in healthcare: past, present and future (Jiang et al. 2018), Conceptualising Artificial Intelligence as a Digital Healthcare Innovation: An introductory Review (Arora, 2020), and Harvard Business Review’s 10 Promising AI Applications in Health Care (Kalis, Collier, Fu, 2018).
